CT2Yarn: Yarn-Level Reconstruction of Crochet from Computed Tomography

We introduce CT2Yarn, a human-in-the-loop framework for recovering a single continuous yarn path from micro-computed tomography (micro-CT) scans of real crochet objects. Crochet is a craft that creates complex three-dimensional shapes by interlocking loops formed from a single yarn. Recovering the underlying yarn path from external observations is challenging because of severe self-occlusion. While micro-CT reveals the full internal structure of a crochet object, the volumetric scan alone does not explicitly encode how the yarn traverses the object. This challenge stems from the hierarchical structure of yarn: a yarn consists of multiple twisted plies, and each ply itself consists of twisted fibers. Consequently, local fiber orientations observed in micro-CT scans are not aligned with the overall yarn direction. To recover yarn-level orientations from ply-level fiber orientations, we first estimate local fiber directions using Gabor filtering and convert the volume into an oriented point cloud. We then introduce an anisotropic mean-shift procedure that aggregates local fiber orientations within a neighborhood of the yarn radius into yarn-level orientation estimates. Combined with an automatic topology skeletonization strategy, our method extracts yarn-path fragments. Subsequent fragment linking, junction cleaning, and loop detection merge these trees into a small number of long curves. Where the automatic reconstruction remains ambiguous, a sketch-based user interface enables users to interactively complete the single continuous yarn path. The recovered yarn path enables downstream applications including physically based simulation, ply-level rendering, and stitch-pattern extraction.

==> secs/_tab_manual.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  % camera-ready: no revision color
  \setlength{\tabcolsep}{2.6pt}
  \begin{tabular}{@{}lrrr@{\hspace{2.2ex}}lrrr@{}}
    \toprule
    Sample & Edits & Time & Len.\,(\%) & Sample & Edits & Time & Len.\,(\%) \\
    \midrule
    Patch 1 & 11 & 2:09 & 1.15 & X & 18 & 4:09 & 2.48 \\
    Patch 2 & 17 & 4:54 & 0.93 & Y & 21 & 5:25 & 3.92 \\
    Patch 3 & 7 & 1:50 & 0.70 & Two (normal) & 24 & 5:24 & 2.05 \\
    G & 21 & 10:35 & 4.49 & Six & 4 & 0:50 & 0.18 \\
    H & 48 & 15:28 & 6.77 & Stick & 15 & 6:42 & 7.47 \\
    O & 6 & 1:37 & 0.99 & Arrow & 23 & 12:28 & 4.57 \\
    P & 11 & 1:31 & 0.29 & & & & \\
    \midrule
    Mean & 14.1 & 4:34 & 2.25 & Median & 13 & 3:09 & 1.07 \\
    \bottomrule
  \end{tabular}
  \caption{\rev{\textbf{Per-sample manual intervention.} Interactive edit operations, editing time (min:s), and the fraction of the final centerline length contributed by manual edits. Samples that required no edits (the three chain-stitch samples) and samples without recorded sessions are omitted from the rows. Mean and median are over the 16 recorded samples.}}
  \label{tab:manual}
\end{table}

